Intent-based Prompt Calibration: Enhancing prompt optimization with synthetic boundary cases

Prompt engineering is a challenging and important task due to the high sensitivity of Large Language Models (LLMs) to the given prompt and the inherent ambiguity of a textual task instruction. Automatic prompt engineering is essential to achieve optimized performance from LLMs. Recent studies have demonstrated the capabilities of LLMs to automatically conduct prompt engineering by employing a meta-prompt that incorporates the outcomes of the last trials and proposes an improved prompt. However, this requires a high-quality benchmark to compare different prompts, which is difficult and expensive to acquire in many real-world use cases. In this work, we introduce a new method for automatic prompt engineering, using a calibration process that iteratively refines the prompt to the user intent. During the optimization process, the system jointly generates synthetic data of boundary use cases and optimizes the prompt according to the generated dataset. We demonstrate the effectiveness of our method with respect to strong proprietary models on real-world tasks such as moderation and generation. Our method outperforms state-of-the-art methods with a limited number of annotated samples. Furthermore, we validate the advantages of each one of the system's key components. Our system is built in a modular way, facilitating easy adaptation to other tasks. The code is available $\href{https://github.com/Eladlev/AutoPrompt}{here}$.

==> git-guide/guide.tex <==


What do we provide?
We provide a system for prompt optimization framework that creates synthetic data

Why choose us?
the system is built for production
tested on real-world use cases 
tested on real-world models, like gpt-4 and gpt




==> old_sections/experiments.tex <==
\section{Experiments}

Returning to our hypothesis from Section \ref{sct:introduction}: \textit{greater prompt-adherence can help address errors and degradations involved in language modeling.} In this section, we explore different variations of prompting tasks, and show that CFG reliably boosts performance. First, we explore the \textit{base-case prompt}, or zero-shot prompt, in Section \ref{sct:experiments:benchmarks}, by applying CFG to a wide range of standard benchmarks, achieving \textit{state-of-the-art} on LLaMa-7b. Next, in Section \ref{sct:experiments:cot}, we test \textit{Chain-of-Thought prompts} \cite{}  an approach to allows the model to reason first before answering the question. Then, we test the performance of CFG on \textit{text-to-text generation prompts} in Section \ref{sct:experiments:text-to-text-generation}, specifically in machine translation and code generation, which involves more direct copying and interpretation of the input. Finally, we show that CFG with \textit{negative prompts}, in Section \ref{sct:experiments:negative-prompting}, can increase control.

\subsection{Basic Prompting: Zero-Shot Prompts}
\label{sct:experiments:benchmarks}

To test \textit{basic, zero-shot prompting}, we consider a suite of zero-shot benchmarks implemented in the Language Model Evaluation Harness \cite{eval-harness}, which includes close-book QA \cite{}, common sense reasoning tasks \cite{}, and sentence completion-tasks \cite{}. In these settings, the desired completions are short (often 1-2 tokens), so risks of meandering \cite{} or degradation \cite{} are low. We hypothesize that the main impact of CFG in these settings will be to reduce variance in output choices, as we explore more in Section \ref{sct:explanation}.

We evaluate the GPT-2 model family\footnote{GPT-2 small, medium, large and xl} (\cite{brown2020language}), the Pythia model family\footnote{Pythia 160M, 410M, 1B, 1.4B, 2.8B, 6.9B and 13B} (\cite{biderman2023pythia}) and the LLaMA model family\footnote{7B, 13B, 30B and 65B} using different guidance strengths across a range of standard NLP benchmarks\footnote{The benchmarks consist of Hellaswag, WinoGrande, Lambada(OpenAI), BoolQ, PIQA, SciQ, ARC-Easy, ARC-Challenge, TriviaQA}. We fork the Language
Model Evaluation Harness (\cite{eval-harness}) and implement CFG by starting the unconditional prompt at the last token of the initial prompt. The results are shown in Table \ref{tab:benchmark}. For better visualization, the charts for the GPT2 models, the Pythia models and the LLaMA models over the standard benchmarks are also shown in Figure \ref{fig:gpt2-split}, \ref{fig:pythia-split}, and \ref{fig:llama-split}, respectively. We observe that except Arc challenge and Winogrande, the boost of performances from CFG is nontrivial and consistent.

Furthermore, we note that even the smallest LLaMA 7B model achieves $81\%$ accuracy in Lambada(OpenAI) zero-shot benchmark with $\gamma = 1.5$, outperforming the current SOTA (zero-shot) of PaLM-540B ($77.9\%$). Despite the fact that CFG almost doubles the computation during inference, the comparison is still noteworthy given that other models with comparable performances on Lambada(OpenAI) have much more parameters and would still require more compute than LLaMA 7B with CFG.

\begin{figure}[t]
    \centering
    \subfloat[][]{
    \begin{tabular}{lllll}
        \toprule
        {} &        ARC-c &        ARC-e &        BoolQ &    HellaSwag \\
        \midrule
        GPT2-xl &   28.5 / \textbf{ 30.0} &   51.1 / \textbf{ 56.5} &   61.8 / \textbf{ 62.6} &   50.9 / \textbf{ 52.4}\\
        GPT2-large &  \textbf{ 25.1} /  24.7 &   46.6 / \textbf{ 51.0} &   60.5 / \textbf{ 62.1} &   45.3 / \textbf{ 47.1}\\
        GPT2-medium &  \textbf{ 25.0} /  23.9 &   43.6 / \textbf{ 47.6} &   58.6 / \textbf{ 60.1} &   39.4 / \textbf{ 40.9}\\
        GPT2-small &   22.7 / \textbf{ 23.0} &   39.5 / \textbf{ 42.1} &   48.7 / \textbf{ 57.0} &   31.1 / \textbf{ 31.9}\\
        \midrule
        Pythia-12B &   36.9 / \textbf{ 38.7} &   64.1 / \textbf{ 72.6} &   67.6 / \textbf{ 67.8} &   67.3 / \textbf{ 69.6}\\
        Pythia-6.9B &   35.2 / \textbf{ 36.1} &   61.3 / \textbf{ 67.4} &   63.7 / \textbf{ 64.6} &   64.0 / \textbf{ 66.5}\\
        Pythia-2.8B &   33.1 / \textbf{ 34.5} &   58.8 / \textbf{ 65.4} &   64.7 / \textbf{ 64.7} &   59.3 / \textbf{ 61.9}\\
        Pythia-1.4B &   28.6 / \textbf{ 29.6} &   53.8 / \textbf{ 59.6} &   63.0 / \textbf{ 63.8} &   52.1 / \textbf{ 54.3}\\
        Pythia-1B &   27.0 / \textbf{ 28.0} &   49.0 / \textbf{ 54.9} &   60.7 / \textbf{ 61.8} &   47.1 / \textbf{ 48.9}\\
        Pythia-410M &  \textbf{ 24.1} /  23.8 &   45.7 / \textbf{ 50.3} &   60.6 / \textbf{ 61.2} &   40.6 / \textbf{ 41.6}\\
        Pythia-160M &  \textbf{ 23.5} /  23.0 &   39.5 / \textbf{ 42.2} &   55.0 / \textbf{ 58.3} &   30.1 / \textbf{ 31.2}\\
        \midrule
        LLaMA-65B &   55.6 / \textbf{ 59.0} &   79.7 / \textbf{ 84.2} &  \textbf{ 84.8} /  83.0 &   84.1 / \textbf{ 86.3}\\
        LLaMA-30B &   52.9 / \textbf{ 57.4} &   78.9 / \textbf{ 83.2} &  \textbf{ 82.7} /  80.0 &   82.6 / \textbf{ 85.3}\\
        LLaMA-13B &   47.8 / \textbf{ 54.2} &   74.8 / \textbf{ 79.1} &  \textbf{ 78.0} /  75.8 &   79.1 / \textbf{ 82.1}\\
        LLaMA-7B &   41.5 / \textbf{ 43.9} &   52.5 / \textbf{ 58.9} &  \textbf{ 73.1} /  71.8 &   73.0 / \textbf{ 76.9}\\

        \bottomrule
    \end{tabular}
    } \\ 
    
    \subfloat[][]{
    \begin{tabular}{llllll}
        \toprule
        {} &         PIQA &         SCIQ &   WinoGrande &      Lambada \\
        \midrule
        GPT2-xl &   70.5 / \textbf{ 71.3} &   76.1 / \textbf{ 82.4} &  \textbf{ 58.3} /  55.6 &   51.2 / \textbf{ 62.5}\\
        GPT2-large &   69.2 / \textbf{ 70.2} &   69.4 / \textbf{ 78.8} &  \textbf{ 55.4} /  54.4 &   47.7 / \textbf{ 60.5}\\
        GPT2-medium &   66.4 / \textbf{ 66.9} &   67.2 / \textbf{ 76.7} &  \textbf{ 53.1} /  52.1 &   43.0 / \textbf{ 55.8}\\
        GPT2-small &   62.5 / \textbf{ 63.8} &   64.4 / \textbf{ 70.8} &  \textbf{ 51.6} /  50.5 &   32.6 / \textbf{ 44.6}\\
        \midrule
        Pythia-12B &   77.0 / \textbf{ 78.4} &   87.7 / \textbf{ 91.9} &  \textbf{ 65.0} /  63.4 &   70.4 / \textbf{ 80.6}\\
        Pythia-6.9B &   76.3 / \textbf{ 77.4} &   84.3 / \textbf{ 89.7} &  \textbf{ 61.1} /  60.3 &   67.1 / \textbf{ 78.8}\\
        Pythia-2.8B &   73.6 / \textbf{ 75.8} &   83.3 / \textbf{ 88.2} &  \textbf{ 60.1} /  57.9 &   64.6 / \textbf{ 76.5}\\
        Pythia-1.4B &   71.1 / \textbf{ 72.5} &   79.4 / \textbf{ 85.1} &  \textbf{ 57.4} /  56.0 &   61.6 / \textbf{ 72.7}\\
        Pythia-1B &   69.2 / \textbf{ 70.5} &   76.0 / \textbf{ 82.9} &  \textbf{ 53.9} /  51.5 &   56.2 / \textbf{ 69.0}\\
        Pythia-410M &   67.1 / \textbf{ 67.8} &   72.1 / \textbf{ 79.0} &  \textbf{ 52.9} /  50.7 &   51.3 / \textbf{ 64.0}\\
        Pythia-160M &   61.4 / \textbf{ 62.1} &   67.0 / \textbf{ 75.4} &  \textbf{ 52.3} /  51.1 &   32.8 / \textbf{ 47.4}\\
        \midrule
        LLaMA-65B &   82.3 / \textbf{ 82.6} &   95.1 / \textbf{ 96.6} &  \textbf{ 77.4} /  76.1 &   79.1 / \textbf{ 84.0}\\
        LLaMA-30B &  \textbf{ 82.3} /  82.3 &   94.3 / \textbf{ 96.4} &  \textbf{ 75.8} /  74.1 &   77.5 / \textbf{ 83.9}\\
        LLaMA-13B &   80.1 / \textbf{ 80.9} &   91.1 / \textbf{ 95.1} &  \textbf{ 72.8} /  71.5 &   76.2 / \textbf{ 82.2}\\
        LLaMA-7B &   77.4 / \textbf{ 79.8} &   66.3 / \textbf{ 75.4} &  \textbf{ 67.1} /  65.5 &   73.6 / \textbf{ 81.3}\\
        \bottomrule
    \end{tabular}
    }
    \caption{Results of general natural language benchmarks. In each cell, the first value is the result for $\gamma = 1$ and the second value is the result for $\gamma = 1.5$.\\LLaMA 7B with CFG on Lambada zero-shot already outperforms vanilla PaLM 540B, Chinchilla 70B, and GPT-3 175B, tops the \href{https://paperswithcode.com/sota/language-modelling-on-lambada}{SOTA leaderboard} for Lambada zero-shot as of June 26th, 2023}
    \label{tab:benchmark}
\end{figure}

Taken together, we show that CFG increases performance in basic prompting settings significantly, and we explore more why in Section \ref{sct:explanation}.

\subsection{Deliberative Prompting: Chain-of-Thought}
\label{sct:experiments:cot}

A variation on \textit{basic prompting} has emerged recently called \textit{Chain-of-Thought (CoT) prompting} \cite{COT}. In this setting, the model is prompted to generate a series of reasoning steps before giving an answer to the task -- i.e. $p(w_c= \left[w_{cot}, w_a\right]| w_p)$, where $w_{cot} = w_{p+1}...w_{c-1}$ and $w_a$ is the answer. $w_{cot}$ is designed to mimic the human reasoning or deliberation process. CoT has been shown to perform well in complex reasoning tasks that could not be fully addressed by model- or data-scaling ~\cite{rae}, however, as observed by~\cite{COT}, long reasoning chains can diverge and either do not generate correct answers, or do not follow the expected result structure given by the prompt.

This setting poses a variation on the prior \textit{base-case} setting: now, the continuation $w_c = \left[w_{cot}, w_{a}\right]$ is expected to be longer than 1-2 tokens. We hypothesize that compared to basic zero-shot prompting explored in Section \ref{sct:experiments:benchmarks}, CFG will \textit{also} be able to enforce better reasoning chains with less drift.

 We evaluate the effectiveness of our proposed CFG method with respect to chain-of-thought prompting on two arithmetic reasoning tasks: GSM8K~\cite{gsm8k} and AQuA~\cite{aqua}. We follow~\cite{self-consistency} few-shot prompt and parsing setting, with respect to two open source LLM models: WizardLM-30B~\cite{xu2023wizardlm} and Guanaco-65B~\cite{guancano}.
As can be seen in Figure~\ref{fig:cot_GSM8K},~\ref{fig:cot_aqua}, using CFG increases the percentage of CoT which results in a valid answer that could be parsed. For low guidance strengths, this results in boosting the model performances. However, for large values, although the model returns more valid results, the quality of the chains is also impacted, and overall the model performances degrade. A qualitative comparison is provided in Table~\ref{tbl:cot_qual1},~\ref{tbl:cot_qual2}.  

\begin{figure}[!ht]
    \includegraphics[width=195pt]{CoT/gsm8k.png}
    \includegraphics[width=195pt]{CoT/guanaco_gsmk.png}
    \caption{CFG impact on chain-of-thought prompting with respect to GSM8K dataset}\label{fig:cot_GSM8K}
\end{figure}

We acknowledge that we have only scratched the surface of exploring CFG's interactions with CoT; for instance, instead of upweighting just $w_p$, we might upweight $w_p, w_{cot}$, or other variations. We anticipate in future work being able to more fully test variations of CFG-weighting on different parts of the CoT process (i.e. $w_p, w_{cot}, w_c$).


\subsection{Text-to-Text Prompts: Generation}
\label{sct:experiments:text-to-text-generation}
In contrast to \textit{basic prompting} and \textit{CoT-prompting}, where we ultimately expect a short answer, $w_a$, many settings require lengthier continuations. In this section, we study two settings, machine translation and code generation, where the quality of answers are highly dependent the ability to stay on target over long sequences of text (both prompt, $w_p$ and continuation, $w_c$). We hypothesize that, in constrast to Sections \ref{sct:experiments:benchmarks} and \ref{sct:experiments:cot}, these tasks require longer-form completions, which CFG's effectiveness in enforcing adherences to many different parts of the prompt. %We also note that previous work \cite{shi2023trusting}. 

\subsubsection{Machine translation}

We evaluate using CFG for machine translation on a variety of models. We choose the WMT14 fr-en \cite{bojar-EtAl:2014:W14-33_wmt14_fr_en} as the dataset of choice to understand if CFG would also help multilingual datasets. We run 0-shot experiments on Bloom-3B \cite{Scao2022BLOOMA1}, a multilingual model trained on 49 languages. We also test on RedPajama-Incite-Base-3B, trained on 1.5T tokens of english text and mT0 \cite{Muennighoff2022CrosslingualGT_mt0} a prompt tuned sequence-to-sequence model. For the Bloom-3B model we also test for multiple prompts and do 1 shot experiments as well. 

We find that for this generation task, $\gamma$ ranging between 1.1 to 1.25 yield the best results and perform increasingly worse at higher values. We additionally observe that the method is prompt-invariant showing gains regardless of the prompt choice in 0-shot performance. We do not see any improvements in the case of 1-shot performance for Bloom-3B. We also do not see any significant performance gains in the case of mT0 suggesting that prompt-tuned models might already be at the pinnacle of possible 0-shot performance.

\begin{table}[t]
    \centering
    \begin{tabular}{lccr} % vertical lines are against NIPS' guidelines
    \toprule     Model    & $\gamma=1$ & $\gamma=1.10$ & $\gamma=1.25$ \\
         \midrule
        Bloom-3B  & $14.16$ & $15.81$ & $14.16$ \\
        RedPajama-Incite-3B & $15.04$ & $17.24$ & $17.78$ \\
        \midrule
                         & $\gamma=1$ & $\gamma=1.05$ & $\gamma=1.10$ \\
        \midrule
        Bloom-3B 1-shot & $29.84$ & $29.19$ & $28.53$ \\
        mT0  & $29.77$ & $29.41$ & $27.79$ \\
        
        \bottomrule
    \end{tabular}
    \caption{Different $\gamma$ for machine translation tasks. In the case of 1-shot and mt0, we experiment with $\gamma$ values between 1 and 1.1 since we see rapid decline at even slightly higher values. All models are evaluated 0-shot unless otherwise specified.}
    \label{tab:mt-gen}
\end{table}



\subsubsection{Program synthesis evaluations}\label{sct:experiments:text-to-text-generation:program_synthesis}
Computer programs represent an important language-modeling case, as formal language differs from natural language in many ways including the use of well-defined structures. Testing CFG on code-related tasks improves the robustness of our hypothesis over different distributions of data. In the exploratory experiments, we prompt GPT-J \cite{gpt-j} and CodeGen-350M-mono \cite{nijkamp2023codegen} for small-scale code generations and observe positive results results \ref{appendix:additional-exp}. And then we perform a thorough evaluation on the HumanEval benchmark \cite{chen2021codex}. 


\subsubsection{HumanEval benchmark}

To systematically investigate the impact of CFG on code completion abilities, we evaluate models using different CFG strengths on HumanEval benchmark (\cite{chen2021codex}). HumanEval benchmark contains $164$ coding tasks in Python where the prompts are given by a function signature and a docstring. The model will generate continuations of the prompt, and the resulting programs will be tested against a set of unit tests for each task which evaluate the correctness of Python programs. We choose CodeGen-350M-mono, CodeGen-2B-mono and CodeGen-6B-mono (\cite{nijkamp2023codegen}) which are specialized in Python program synthesis. \textit{Note: CodeGen-16B-mono is omitted due to the compute constraint.}

Various CFG strengths \footnote{$\gamma = 1.0, 1.1, 1.25, 1.5, 1.75, 2.0$} are tested on $3$ different temperatures $0.2, 0.6, 0.8$ with the evaluation metrics being pass@$k$ for $k=1, 10, 100$ \footnote{The definition of pass@$k$ according to \cite{chen2021codex}: ``$k$ code samples are generated
per problem, a problem is considered solved if any sample passes the unit tests, and the total fraction of problems
solved is reported."}. The full results are summarized in the Table \ref{tab:codegen-350}, \ref{tab:codegen-2b} and \ref{tab:codegen-6b}. For better visualization, plots for the results of CodeGen-350M-mono, CodeGen-2B-mono and CodeGen-6B-mono are shown in the appendix in Figure \ref{fig:codegen350}, \ref{fig:codegen2b} and \ref{fig:codegen6b}, respectively.

\begin{table}[t]
    \centering
    \begin{tabular}{llllllllll}
        \toprule
         & \multicolumn{3}{c}{temperature = 0.2} & \multicolumn{3}{c}{temperature = 0.6} & \multicolumn{3}{c}{temperature = 0.8} \\
         \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
        $\gamma$ & k=1 & k=10 & k=100 & k=1 & k=10 & k=100 & k=1 & k=10 & k=100 \\
        \midrule
        1.0 & 11.0\% & 17.0\% & \textbf{22.0\%} & 8.9\% & 18.2\% & 23.7\% & 7.2\% & 17.2\% & \textbf{29.4\%} \\
        1.1 & \textbf{11.8\%} & \textbf{18.1\%} & 20.1\% & \textbf{10.0\%} & \textbf{19.7\%} & \textbf{25.5\%} & 7.8\% & 17.1\% & 22.5\% \\
        1.25 & 11.4\% & 17.3\% & 18.9\% & 9.7\% & 18.4\% & 23.7\% & \textbf{8.3\%} & \textbf{18.2\%} & 24.9\% \\
        1.5 & 10.9\% & 16.7\% & 18.3\% & 9.9\% & 19.3\% & 24.9\% & 8.0\% & 18.0\% & 26.1\% \\
        1.75 & 10.3\% & 16.0\% & 18.2\% & 9.2\% & 18.3\% & 23.7\% & 7.7\% & 16.9\% & 24.2\% \\
        2.0 & 8.6\% & 14.6\% & 17.6\% & 7.6\% & 16.6\% & 20.1\% & 7.4\% & 16.5\% & 21.3\% \\
        \bottomrule
    \end{tabular}
    \caption{CodeGen-350M-mono results}
    \label{tab:codegen-350}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{llllllllll}
        \toprule
         & \multicolumn{3}{c}{temperature = 0.2} & \multicolumn{3}{c}{temperature = 0.6} & \multicolumn{3}{c}{temperature = 0.8} \\
         \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
        $\gamma$ & k=1 & k=10 & k=100 & k=1 & k=10 & k=100 & k=1 & k=10 & k=100 \\
        \midrule
        1.0 & 19.5\% & 25.5\% & \textbf{29.8\%} & 15.9\% & 29.3\% & 36.5\% & 12.3\% & 26.4\% & 33.5\% \\
        1.1 & 20.4\% & 25.4\% & 28.0\% & 16.3\% & 29.3\% & 36.5\% & 13.8\% & 29.0\% & \textbf{38.3\%} \\
        1.25 & 19.7\% & 25.4\% & 28.0\% & 17.4\% & 30.1\% & 38.3\% & 14.1\% & 28.7\% & 37.6\% \\
        1.5 & \textbf{20.9\%} & \textbf{26.7\%} & 29.2\% & \textbf{18.3\%} & \textbf{31.7\%} & \textbf{40.1\%} & \textbf{14.9\%} & \textbf{29.1\%} & 36.5\% \\
        1.75 & 20.4\% & 26.2\% & 28.6\% & 17.7\% & 30.4\% & 35.9\% & 14.3\% & 28.3\% & 34.1\% \\
        2.0 & 16.5\% & 22.4\% & 24.4\% & 13.7\% & 25.2\% & 32.2\% & 11.3\% & 23.9\% & 31.6\% \\
        \bottomrule
    \end{tabular}
    \caption{CodeGen-2B-mono results}
    \label{tab:codegen-2b}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{llllllllll}
        \toprule
        & \multicolumn{3}{c}{temperature = 0.2} & \multicolumn{3}{c}{temperature = 0.6} & \multicolumn{3}{c}{temperature = 0.8} \\
         \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
        $\gamma$ & k=1 & k=10 & k=100 & k=1 & k=10 & k=100 & k=1 & k=10 & k=100 \\
        \midrule
        1.0 & 19.5\% & 25.5\% & \textbf{29.8\%} & 15.9\% & 29.3\% & 36.5\% & 12.3\% & 26.4\% & 33.5\% \\
        1.1 & 20.4\% & 25.4\% & 28.0\% & 16.3\% & 29.3\% & 36.5\% & 13.8\% & 29.0\% & \textbf{38.3}\% \\
        1.25 & 19.7\% & 25.4\% & 28.0\% & 17.4\% & 30.1\% & 38.3\% & 14.1\% & 28.7\% & 37.6\% \\
        1.5 & \textbf{20.9\%} & \textbf{26.7\%} & 29.2\% & \textbf{18.3\%} & \textbf{31.7\%} & \textbf{40.1\%} & \textbf{14.9\%} & \textbf{29.1\%} & 36.5\% \\
        1.75 & 20.4\% & 26.2\% & 28.6\% & 17.7\% & 30.4\% & 35.9\% & 14.3\% & 28.3\% & 34.1\% \\
        2.0 & 16.5\% & 22.4\% & 24.4\% & 13.7\% & 25.2\% & 32.2\% & 11.3\% & 23.9\% & 31.6\% \\
        \bottomrule
    \end{tabular}
    \caption{CodeGen-6B-mono results}
    \label{tab:codegen-6b}
\end{table}

We observe that low CFG ($\gamma \leq 1.5 $) increases the pass@$1$ rate uniformly\footnote{Note that the effect of low CFG on the pass@$1$ rate is consistent with the results of the general benchmarks in the previous section.}. High CFG ($\gamma \geq 1.5$) leads to a deterioration of performance. We also note that the improvement from CFG diminishes, or harms performance at pass@$k$ when $k$ is high.

To further investigate the effect of CFG, we break down the pass@$1$ evaluations on CodeGen-350M-mono for $\gamma = 1, 1.25$ task-by-task \footnote{See the scatter plot at temperature $0.2, 0.6, 0.8$ in appendix, Figure \ref{fig:humaneval-tasks-0.8}, \ref{fig:humaneval-tasks-0.6}, \ref{fig:humaneval-tasks-0.2}}. We notice that the number of tasks where CFG outperforms is still more than the one where CFG underperforms for all temperatures $0.2, 0.6, 0.8$ (See Table \ref{tab:codegen-350-task-count}). 

\begin{table}[t]
    \centering
    %\begin{tabular}{llll}
    %\toprule
    %     &  temp = $0.2$ & temp = $0.6$ & temp = $0.8$ \\
    %     \midrule
    %    CFG outperforms & 20 & 24 & 34 \\
    %    CFG underperforms & 18 & 16 & 23 \\
    %    ties\tablefootnote{The majority of them have $0\%$ rate for both $\gamma$} & 126 & 124 & 107 \\
    %    \bottomrule
    %\end{tabular}
    \includegraphics[width=300px]{codegen_350m_charts/task_count.png}
    \caption{HumanEval task count comparison between $\gamma = 1, 1.25$ for CodeGen-350M-mono}
    \label{tab:codegen-350-task-count}
\end{table}

We also find that without CFG, many tasks exhibit small nonzero passing rates while having $0\%$ rate with CFG. This explains the decreasing improvement of CFG in pass@$k$ for large $k$, as larger $k$ significantly boosts the passing rate of difficult tasks where the rates are low but nonzero.

Overall, the consistent improvement on pass@$1$ rates and the reduced effect on pass@$100$ rates support our hypothesis that CFG strengthens the adherence to the prompt at the small cost of reduced variability and creativity.

\subsection{Negative Prompting: Improving Assistants}
\label{sct:experiments:negative-prompting}

Finally, we explore an addition to CFG called \textit{negative prompting}, derived from text-to-image. With negative prompting, the user specifies what they do \textit{not} want in the output (e.g. ``low resolution'', ``bad hands, bad anatomy, amateur drawing''), which is then used to improve generation quality.

We explore this idea in the context of chatbots. Chatbots give us a setting where the \textit{prompt} is expanded into a \textit{multi-stage prompt} (in contrast to \textit{CoT-prompting} in Section \ref{sct:experiments:cot} where the \textit{continuation} was expanded into a \textit{multi-stage completion}). In chatbots, the language model is prompted with a two-part prompt: (1) the instruction, $w_s$ (sometimes called "system prompt") which may give contextual information (e.g. the ``current date''), or behavioral guidelines (e.g. style, alignment, persona, etc.); and (2) $w_p$, the user-prompt, or the user's query. See Table \ref{tbl:example} for an example. Adherence becomes an even greater challenge, as our initial explorations shows. We observe systems like Alpaca \cite{alpaca,vicuna,gpt4all} often ignore changes to their default system-prompt, and may even expose models to attacks like prompt injection \cite{greshake2023more}. 

%PREVIOUSLY: In the previous sections, the prompt was set as a basis to evaluate the relevance of its natural continuation. In chatbots however, it follows a different format and purpose, allowing us to evaluate CFG in a qualitatively different situation. The prompt is composed of two parts: (1) the instruction, $w_s$ (sometimes called "system prompt") which is set by the developer and may give the agent contextual information (e.g. the current date or weather), or behavioral guidelines for the generative process (e.g. style, alignment, persona, abilities, etc.); and (2) $w_p$, the user-prompt, or the user's query which is similar to a standard prompt in the \textit{basic-prompting} case. See Table \ref{tbl:example} for an example of such a setup.  We notice that current chatbots like Alpaca \cite{alpaca,vicuna,gpt4all} all use a default neutral system prompt \footnote{namely: ``The prompt below is a question to answer, a task to complete, or a conversation to respond to; decide which and write an appropriate response.''} whose variations were often ignored by the model in our early experiments.

We explore CFG with negative prompting as a mean to increase the success rate of different system prompts. We set the negative prompt $\overline{c}$ to be the default prompt (``The prompt below is a question to answer, a task to complete, or a conversation to respond to; decide which and write an appropriate response.'') and set $c$ to be the edited prompt (e.g. ``The prompt below is a question to answer, a task to complete, or a conversation to respond to; decide which and write \textit{a sad} response.'').

Where $w_p$, $w_i$ are defined above, and $\overline{w_i}$ is a \textit{different} prompt\footnote{we use the default (neutral) system-prompt: EXAMPLE)}. This approach not only makes the sampling more prompt-aware in general, but directly emphasizes an attribute that we do not want in the output. 

To test negative prompting with chatbots, we generate system-prompts, $n_{c} = 25$, and user-prompts, $n_{p} = 46$, and sample $1740$ random combinations of them. An example is shown in Table \ref{tbl:example} (in Appendix \ref{} we include the full list of $c$ and $p$ we use). We use \texttt{GPT4All-J v1.3-jazzy} to generate two completions for each sampled combination. For each pair, one is sampled without CFG, and guidance strength is randomly chosen in {1,2,3,4,5,6} for the second. Our hypothesis is that CFG increases system-prompt following, ideally without hurting the relevance to the user input. 

We run a human preference study where participants are shown (1) our output and (2) the vanilla GPT4All output and asked to assess two things. A. Which output better follows the system-prompt, $c$ and B. which output better follows the user-prompt $p$. Our results in Figure \ref{fig:gpt4all-human} shows compelling evidence that CFG emphasized the difference between $c$ and $\overline{c}$ more than sampling with $c$ alone. There is a clear peak at $\gamma=3$ with 75\% of system-prompt following preference over $\gamma=1$ and undegraded user-prompt relevance (52\%). 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{gpt4all.png}
    \caption{The evaluators (611 votes, 71 unique voters) consistently and significatively preferred the system-prompt following of $\gamma>1$ with a peak at $\gamma=3$, subject to CFG. The user-prompt relevance, not subject to CFG, did not degrade until $\gamma\ge 4$, showing a clear win without any tradeoff at $\gamma=3$.}
    \label{fig:gpt4all-human}
\end{figure}

\begin{figure}
    \centering
    \subfloat[Entropy of logits for the vanilla prompted distribution $p(y|x)$, the unprompted distribution, $p(x)$, the CFG-$\gamma=1.5$ distribution and an instruction-tuned model $p_{instruct}(y|x)$.]{\includegraphics[width=.5\linewidth]{explanation/entropy.png}
    \label{fig:entropy}
    }
    \subfloat[Number of tokens overlapping in top-p=90\% of vocabulary distributions between that of: CFG, that of the vanilla prompted model, $p(y|x)$, and that of the unprompted model, $p(x)$.]{\includegraphics[width=.5\linewidth]{explanation/p_cfg__token_overlap.png}
    \label{fig:topp}}
    \caption{We give insight into how CFG alters the logit distribution of the vanilla prompted model, $p(y|x)$. We find that CFG lowers the entropy to a level roughly similar to instruction-tuned model variant. CFG shares roughly 50\% of the tokens in $top-p=.9$ as the vanilla $p(y|x)$ model.}
    \label{fig:single-model-comparisons}
\end{figure}

